Make Large Language Model a Better Ranker

Large Language Models (LLMs) demonstrate robust capabilities across various fields, leading to a paradigm shift in LLM-enhanced Recommender System (RS). Research to date focuses on point-wise and pair-wise recommendation paradigms, which are inefficient for LLM-based recommenders due to high computational costs. However, existing list-wise approaches also fall short in ranking tasks due to misalignment between ranking objectives and next-token prediction. Moreover, these LLM-based methods struggle to effectively address the order relation among candidates, particularly given the scale of ratings. To address these challenges, this paper introduces the large language model framework with Aligned Listwise Ranking Objectives (ALRO). ALRO is designed to bridge the gap between the capabilities of LLMs and the nuanced requirements of ranking tasks. Specifically, ALRO employs explicit feedback in a listwise manner by introducing soft lambda loss, a customized adaptation of lambda loss designed for optimizing order relations. This mechanism provides more accurate optimization goals, enhancing the ranking process. Additionally, ALRO incorporates a permutation-sensitive learning mechanism that addresses position bias, a prevalent issue in generative models, without imposing additional computational burdens during inference. Our evaluative studies reveal that ALRO outperforms both existing embedding-based recommendation methods and LLM-based recommendation baselines.

==> section/response.tex <==
\section*{Response to Reviewer Comments and Revision of the Paper}

We appreciate the valuable feedback provided by the reviewers. Below are our detailed responses to the suggestions and the corresponding revisions made to the paper:

\begin{enumerate}
    \item \textbf{Limited Technical Contribution} \\
    To address this issue, we have added more description in Section 2.1, highlighting that existing work focuses on naive supervised fine-tuning, which is ineffective when managing the order relation among candidates. And we point out the importance of introducing out learning framework that could handle the magnitude of the rating. Additionally, in Section 4.3, we demonstrate why lambda loss cannot be directly applied to natural language generation tasks and how it is effective in explicit feedback scenarios.
    
    \item \textbf{Experimental Settings Unclear} \\
    We have clarified the explicit feedback ranking setting in Section 5.1 to ensure the reproducibility of our model. Additionally, we have redone all experiments based on the updated settings as discussed in Section 5.

    \item \textbf{Limited Datasets} \\
    In response to this suggestion, we have introduced three additional updated datasets from Amazon. The details of these datasets and their inclusion in our experiments are elaborated in Section 5.1.

    \item \textbf{Details on Permutation-Sensitive Loss} \\
    We have updated our method for measuring the distance between two output distributions and provided comprehensive details of this method in Appendix~\ref{appendix:PSL}.

    \item \textbf{Missing Baseline Methods} \\
    We have addressed this concern by including additional baseline methods in our experiments in Section 5.2. The specifics of these baselines and their performance comparisons are detailed within the revised sections of the paper.

\end{enumerate}

Furthermore, we have refined our argument to emphasize that existing LLM-based methods predominantly utilize implicit feedback, whereas explicit feedback can significantly contribute to the ranking task. Our proposed framework demonstrates superior performance compared to the baseline methods in this ranking problem.

We hope these revisions meet the reviewers' expectations and enhance the clarity of our paper. Thank you for your constructive feedback.
